Explainable Agents Through Social Cues: A Review

The issue of how to make embodied agents explainable has experienced a surge of interest over the last three years, and, there are many terms that refer to this concept, e.g., transparency or legibility. One reason for this high variance in terminology is the unique array of social cues that embodied agents can access in contrast to that accessed by non-embodied agents. Another reason is that different authors use these terms in different ways. Hence, we review the existing literature on explainability and organize it by (1) providing an overview of existing definitions, (2) showing how explainability is implemented and how it exploits different social cues, and (3) showing how the impact of explainability is measured. Additionally, we present a list of open questions and challenges that highlight areas that require further investigation by the community. This provides the interested reader with an overview of the current state-of-the-art.

==> definitions_table.tex <==
\citet{akash2018a} & Provide visual, context-dependentrecommendations based on the levelof trust and workload of the human & Trust,  Human’s  Workload,  Real-Time Human-Robot Collaboration,Recommendation, Visualization, In-formed Judgements \\\\
\citet{akash2019}b & Provide visual, context-dependentrecommendations based on the levelof trust and workload of the human & Trust,  Human’s  Workload,  Real-Time Human-Robot Collaboration,Recommendation, Visualization, In-formed Judgements \\\\
\citet{baraka2018b} & Externalize hidden information ofan agent. Express robot behaviorsthat have a specific communicativepurpose. & Human-Robot Collaboration, Con-trol, Communication \\\\
\citet{boyce2015} & Display transparency information(SAT model {[}16{]}) in the interface ofan autonomous robot & Trust \\\\
\citet{chakraborti2017} & Identify and reconcile the relevantdifferences  between  the  humans’and robot’s model for building op-timal explanations. Reveal informa-tion regarding the future intentionsof the robot at the time of task exe-cution using projection-aware plan-ning & Communication, Human-Robot Col-laboration, Impedance Mismatch \\\\
\citet{chakraborti2018a} & Identify and reconcile the relevantdifferences  between  the  humans’and robot’s model for building op-timal explanations. Reveal informa-tion regarding the future intentionsof the robot at the time of task exe-cution using projection-aware plan-ning & Communication, Human-Robot Col-laboration, Impedance Mismatch \\\\
\citet{chao2010} & Explain the robot’s internal statesin order to improve the learning ex-perience by revealing to the teacherwhat is known and what is unclear & Machine Teaching, Predictability \\\\
\citet{chen2017} & Visualize intent, reasoning and pre-dicted   future   states   (perception,comprehension and projection) & Trust, Human’s Workload \\\\
\citet{floyd2016} & SAT model &  \\\\
\citet{floyd2017} & SAT model &  \\\\
\citet{gong2018} & Signal intentions using natural lan-guage & Teamwork, Human-Robot Collabo-ration \\\\
\citet{hayes2017} & Share expectations and mutual un-derstanding in human-robot collab-orative contexts. Convey intentions,plans, or justifications & Control, Debug \\\\
\citet{huang2019} & Communicate  information  to  cor-rectly anticipate a robot’s behaviorin novel situations and building anaccurate mental model of the robot’sobjective function & Prediction, Human-Robot Coordina-tion \\\\
\citet{khoramshai2019} &  &  \\\\
\citet{kwon2018} & Express  robot’s  incapability  andcommunicate both what the robotis trying to accomplish and why therobot is unable to accomplish it & Robot’s Acceptance, Human-RobotCollaboration \\\\
\citet{lamb2018} & Implement behavioral dynamics models based on human decision-making dynamics & Human-Robot Collaboration \\\\
\citet{lee2010} & unspecified &  \\\\
\citet{legg2019} & Establish a two-way collaborative dialogue on data attributions between human and machine and express personal confidence in data attributions & Active Learning, Human-Robot Collaboration \\\\
\citet{lutkebohle2009} & Structure verbal and non-verbal di-alog to guide human actions & Machine  Teaching,  Predictability,Human-Robot Collaboration \\\\
\citet{perlmutter2016} & Communicate robot’s internal pro-cesses with human-like verbal andnon-verbal behaviors & Communication, Visualization, Con-trol \\\\
\citet{poulsen2019} & Real-time graphical and audible rep-resentation for communicating therobot’s decision-making processesand reflecting on the robot’s real ca-pabilities, intentions, goals and limi-tations & Ethical Decision-Making, Trust \\\\
\citet{roncone2017} & Provide appropriate measures of un-certainty  for  having  mental  mod-els about the tasks shared betweenpeers & Trust, Proficiency, Confidence, Un-certainty, Introspection \\\\
\citet{schaefer2016} & Visualize robot’s reasoning pro-cesses and intent & Human-Robot Collaboration, Trust \\\\
\citet{sciutti2014} & Convey cues about object features(e.g., weight) to the human partnerusing implicit communication & Human-Robot Collaboration \\\\
\citet{sheikholeslami2018} &  &  \\\\
\citet{sreedharan2017} & Produce a plan that is closer to thehuman’s expected plan and a planexplanation that includes correctionof the belief state (goals or state in-formation) as well as informationpertaining to the action model itself & Human-Aware  Planning,  Human-Robot Collaboration \\\\
\citet{tabrez2019} & Anticipate,  communicate,  and  ex-plain justifications and rationale forAI driven behaviors via contextuallyappropriate semantics & Trust, Machine Teaching \\\\
\citet{wang2016a} & Generate  explanations  of  the  ro-bot’s reasoning, communicate un-certainty and conflicting goals & Trust, Teamwork \\\\
\citet{wang2016b} & Generate explanations of the robot's reasoning, communicate uncertainty and conflicting goals & Trust, Teamwork \\\\
\citet{wang2018} & Generate explanations of the robot's reasoning, communicate uncertainty and conflicting goals & Trust, Teamwork \\\\
\citet{zhou2017} & Communicate the robot’s internalstate though timing & Perceived Naturalness, Human’s Learning (Task Understanding)

==> tab_methods.tex <==
\begin{landscape}
\begin{longtable}{p{2cm}p{3.5cm}p{3.5cm}p{3.5cm}p{3.5cm}}
\caption{Explanability Mechanisms used in different tasks}
\label{tab:algorithms} \\
\toprule
\textbf{Author(s)} & \textbf{Task} & \textbf{Goal} & \textbf{Agent Algorithm} & \textbf{Explainability Algorithm}\\
\midrule
\endfirsthead
\toprule
\textbf{Author(s)} & \textbf{Task}  & \textbf{Goal} & \textbf{Agent Algorithm} & \textbf{Explainability Algorithm}\\
\midrule
\endhead
\bottomrule
\endfoot
\bottomrule
\endlastfoot

\citet{lutkebohle2009} & Explain to a robot affordances of objects (name and graspability) & Facilitate efficient learning through mixed-initiative dialog & custom system based on the XCF toolkit focusing on perceptual analysis, task generation, and dialog-oriented generation & Not specified\\ 

\citet{chao2010} & Teach Simon robot the meaning of four words & Recognition of paired configurations of objects & Supervised Learning & Active Learning to query a human teacher about a demonstration within the context of a social dialogue \\ \\

\citet{lee2010} & Evaluate robots response (forwarning and style of recovery) on a hypothetical scenario & Create a better service experience for users of a snack selling robot & None & Static explanation based on assigned condition\\\\

\citet{lee2013} & Evaluate robots response (forwarning and style of recovery) on a hypothetical scenario & Discover changes in trust based on participant's understanding of a robot's decision making process & None & None \\\\

\citet{sciutti2014} & Observe motion of iCub robot & Investigate if robot motion can be understood in the same way as human movement & Static display of robot behavior & static display of explainability queues  \\\\

\citet{boyce2015} & Observe a virtual agent moving around in a simulated environment & Assess the amount of trust elicited by the system based on the degree of explainability shown & Not specified & Different levels of static explainability mechanisms based on experimental condition\\\\

\citet{perlmutter2016} & Instruct a PR-2 robot to pick and place objects & Assess if screen or VR headset is useful to provide users with information on how the robot works internally & Simulated language understanding & Static display of explainability queues\\\\

\citet{floyd2016, floyd2017} & Issue commands and monitor robot behavior in a virtual patrol scenario & Use explainable behavior for adaptation & Behavior adaptation using probabilistic methods & Select feedback based on how closely current behavioral change matches past behavioral change where this explanation was used\\\

\citet{chen2017} & Study 1: simulation of an autonomous squat member providing information support, Study 2: participants rated abstract plans to complete different missions & Enable users to accurately assess a situation and calibrate their trust in the system while balancing workload & Not specified & Static explanation based on assigned condition\\ \\

\citet{schaefer2016} & Sit in a drive simulator for an autonomous car and perform a taxi/chauffeur task & Increase user trust in driverless cars & Not specified & Not specified\\\\

\citet{wang2016b} & Simulated recon mission where human and robot search buildings for potential threats & Dynamically generate explanations to maintain user's trust in an unreliable system & Use PsychSim to generate a belief of the world (using a POMDP) that is updated based on the user's actions & Use natural-language templates to convert POMDP state into explanation\\\\

\citet{wang2016a} & Simulated recon mission where human and robot search buildings for potential threats & Participants collaborate with autonomous robot in recon mission & Reinforcement learning on POMDP & Static addition of robot's confidence in prediction\\\\

\citet{hayes2017} & Simulation of a grid-world delivery task, inverse pendulum, and part inspection task & Delivery Task, Stabilization Task, Inspection task & Mapping an action query to a policy explanation, MDPs representation, Collection of Boolean classifiers (communicable predicates) to provide meaningful abstraction over low-level information & Autonomously synthesize robot policy descriptions and respond to both general and targeted queries by human collaborators \\\\

\citet{zhou2017} & Observe motion of 6DoF actuator & Create transparent robot motion & Static display of robot behavior & Static display of transparency queues \\\\

\citet{roncone2017} & Joint construction of flat-pack furniture & Reduce workload for human and make overall task more efficient & POMDP-planner & Not specified explicitly\\\\

\citet{chakraborti2017} & Review proposed plan to solve a maze and assess the optimality of it & Evaluate explanation generation algorithms & None & Selection of human generated explanation database by category \\\\

\citet{sreedharan2017} & Humans observe the agent's plan presented on a map and judge it's optimality & Provide explanations that help humans understand why robot plan is optimal & Tree search exploring the domain's graph & MEGA algorithm \\ 

\citet{gong2018} & observe robot performing various household maintenance tasks in a simulated apartment & Generate natural language explanations of robot intent & Not specified & Probabilistic algorithm to select utterance and timing of utterance\\\\

\citet{kwon2018} & Observe virtual robot fail to perform a series of tasks and assess the reason for failure; tasks: lift, push, pull, pull down, push sideways & Make the reason for incapability aparent to observer & Standard motion planning & Custom cost function and distance metrics in planner\\\\

\citet{poulsen2018} & Evaluate robot behavior in a hypothetical interaction scenario between a robot and caregiver & Discover changes in trust based on participant's understanding of a robot's decision making process & None & None \\\\

\citet{baraka2018b} & Observe LED lights on robot to infer robot's internal state & Allow robot to communicate it's state efficiently & CoBot stack & Algorithm to select expressive animation based on current robot state\\\\

\citet{lamb2018} & Collaborative pick and place task, where human and robot perform a handover to move an object & Establish smooth handover behaviors between robots and humans & Model based closed loop controller & Use the proposed control algorithm with specific parameters to achieve human like behavior \\\\

\citet{sheikholeslami2018} & Study 1: humans were asked to pack items into a box; Study 2: Humans observe a robot packing items into a box based on the model learned from study 1 & Generate human interpretable reaching behaviors & Motion planner & Setting the parameters using parameter estimation from mocap experiment \\\\

\citet{akash2018a} & Simulated recon mission where human and robot search buildings for potential threats & Investigate influence of transparency on trust in the system & None & Static explanation based on assigned condition \\\\

\citet{akash2018b} & Simulated recon mission where human and robot search buildings for potential threats & Validate the proposed algorithm for choosing explanations & Not specified & Leverage POMDP-based trust and workload model to choose type of explanation to be provided in each consecutive scenario \\\\

\citet{huang2019} & Observe a simulated autonomous car driving on a road &  Allow human observers to deduce robot's objective function more quickly & Static example behaviors & Model human understanding as inverse reinforcement learning problem\\\\

\citet{tabrez2019} & Collaborative puzzle game inspired by Sudoku, where both players arrange colors in a grid while adhering to constraints & Assess utility of explanation when detecting errors in human behavior & RARE: Reward Augmentation and Repair through Explanation based on Partially Observable Markov Decision Process (POMDP) and Hidden Markov Models (HMMs) & estimate collaborator's reward function during joint task execution and use communicative action if model differs from robot's model \\ \\

\citet{legg2019} & Humans and machines jointly label a dataset to improve prediction accuracy of ML model & Improve sample efficiency of ML algorithm & Different machine learning algorithms combined with various metrics to select samples for labeling & Static display of transparency queues\\\\

\citet{khoramshai2019} & Scenario 1: manipulation task where assists user processing a piece of wood; Scenario 2: robot and user are jointly carrying a heavy object & Intelligently and compliantly adapt motion to the intention of the human & Behavior adaptation algorithm that smoothly blends between behaviors based on human input & None\\\\

\bottomrule
\end{longtable}
\end{landscape}

